MOCHA: Real-Time Motion Characterization via Context Matching

Transforming neutral, characterless input motions to embody the distinct style of a notable character in real time is highly compelling for character animation. This paper introduces MOCHA, a novel online motion characterization framework that transfers both motion styles and body proportions from a target character to an input source motion. MOCHA begins by encoding the input motion into a motion feature that structures the body part topology and captures motion dependencies for effective characterization. Central to our framework is the Neural Context Matcher, which generates a motion feature for the target character with the most similar context to the input motion feature. The conditioned autoregressive model of the Neural Context Matcher can produce temporally coherent character features in each time frame. To generate the final characterized pose, our Characterizer network incorporates the characteristic aspects of the target motion feature into the input motion feature while preserving its context. This is achieved through a transformer model that introduces the adaptive instance normalization and context mapping-based cross-attention, effectively injecting the character feature into the source feature. We validate the performance of our framework through comparisons with prior work and an ablation study. Our framework can easily accommodate various applications, including characterization with only sparse input and real-time characterization. Additionally, we contribute a high-quality motion dataset comprising six different characters performing a range of motions, which can serve as a valuable resource for future research.

==> Sections/7_Limitation_and_future_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion and Conclusion}%{Limitation and Future work}
\label{sec:limitation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
%SH: remove to save space. show them in video instead.
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\linewidth]{Figures/limitation.png}
  \caption{Failure cases.}
  \label{fig:limtation}
\end{figure}
\end{comment}

We introduced MOCHA, a motion characterization framework that can transform user motions to embody distinct style of characters in real-time, and demonstrated its effectiveness through a number of experiments and analysis.

Our method has several limitations that necessitates further exploration.
First, our method is most effective when a character motion dataset contains a single characteristic style per context. If multiple motions with different styles share the same context for a target character, our NCM may encounter difficulties in generating temporally consistent character features, leading to discontinuous motions. We observed such phenomena when consolidating all emotion sets of a character into one, thereby allowing emotional style variations within the same motion. Future work is needed to enable such style variations even within a single character.

Second, while our unsupervised learning of context mapping is effective without manual style labels, it is not flexible enough to encompass all stylistic diversity of the character data.
For instance, Angry Ogre motions in our database has a unique style of running on all fours and jumping sideways. Our algorihtm currently could not link them to the running and jumping motions of other characters, as shown in the supplementary video. More advanced methods for context learning is desirable to improve the characterization quality.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Acknowledgement}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{acks}
This work was conducted during Deok-Kyeong Jang's internship at Meta. Deok-Kyeong Jang would like to thank Michelle Hill for her help in capturing the dataset and the Meta team for their mentorship and support during his internship. Jungdam Won was partially supported by the New Faculty Startup Fund from Seoul National University, ICT (Institute of Computer Technology) at Seoul National University. Sung-Hee Lee was partially supported by the Technology Innovation Program (20011076) of KEIT.
\end{acks}
